High Fidelity Speech Enhancement with Band-split RNN

Despite the rapid progress in speech enhancement (SE) research, enhancing the quality of desired speech in environments with strong noise and interfering speakers remains challenging. In this paper, we extend the application of the recently proposed band-split RNN (BSRNN) model to full-band SE and personalized SE (PSE) tasks. To mitigate the effects of unstable high-frequency components in full-band speech, we perform bi-directional and uni-directional band-level modeling to low-frequency and high-frequency subbands, respectively. For PSE task, we incorporate a speaker enrollment module into BSRNN to utilize target speaker information. Moreover, we utilize a MetricGAN discriminator (MGD) and a multi-resolution spectrogram discriminator (MRSD) to improve perceptual quality metrics. Experimental results show that our system outperforms various top-ranking SE systems, achieves state-of-the-art (SOTA) results on the DNS-2020 test set and ranks among the top 3 in the DNS-2023 challenge.

==> abstract.tex <==
\begin{abstract}
Despite the rapid progress in speech enhancement (SE) research, enhancing the quality of desired speech in environments with strong noise and interfering speakers remains challenging.
In this paper, we extend the application of the recently proposed band-split RNN (BSRNN) model to full-band SE and personalized SE (PSE) tasks.
To mitigate the effects of unstable high-frequency components in full-band speech, we perform bi-directional and uni-directional band-level modeling to low-frequency and high-frequency subbands, respectively. 
For PSE task, we incorporate a speaker enrollment module into BSRNN to utilize target speaker information.
Moreover, we utilize a MetricGAN discriminator (MGD) and a multi-resolution spectrogram discriminator (MRSD) to improve perceptual quality metrics. 
Experimental results show that our system outperforms various top-ranking SE systems, achieves state-of-the-art (SOTA) results on the DNS-2020 test set and ranks among the top 3 in the DNS-2023 challenge.

% In this paper, we broaden the application of the band-split RNN (BSRNN), a frequency-domain source separation model recently proposed, to encompass the tasks of speech enhancement and personalized speech enhancement.


% This report presents the development of Tencent AI Lab's personalized speech enhancement system for the ICASSP 2023 deep noise suppression (DNS) challenge, 
% which includes the use of a modified band-split recurrent neural network (BSRNN) and a multi-frequency discriminator to improve the perceptual quality metrics such as personalized DNSMOS P.835 (PDNSMOS). 
% The proposed system outperforms the baseline system by 0.047 and 0.036 final scores in the headset track and speaker phone track, respectively, and ranks the 3rd in both tracks. 
\end{abstract}
\begin{keywords}
Full-band speech enhancement, Personalized speech enhancement, Band-split RNN
\end{keywords}

==> bak.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% File:     INTERSPEECH2023.cls % class file for INTERSPEECH2023
%
% Usage:    \documentclass{INTERSPEECH2023}
%
% Purpose:
%
% Style file for INTERSPEECH 2023 Conference.
% Modified from previous INTERSPEECH conferences
% Features:
%    - correct page size (175mm x 226mm)
%    - use Times-Roman font as default font (roman font) in order to achieve
%      best quality on paper and screen
%    - two-column format
%    - boldfaced, numbered, and centered section headings
%    - correct subsection and subsubsection headings
%    - \sloppy is now the default but can be changed to \fussy by
%      specifying it as a package option (i.e. \usepackage[fussy]{INTERSPEECH})
%    - use \title{xx} for title, will be typeset all uppercase
%    - use \name{xx} for author name(s) only, will be typeset in italics
%    - use \address{xx} for authors' affiliations, one per line
%    - use \email{xx} for authors' email addresses, will be typeset
%      in proportional typeface
%    - note: no need for \author nor \date
%    - optional: can use \thanks{xx} within \name, asterisk is
%      not printed after name nor in footnote
%    - optional: can use \sthanks{xx} after each name within \name,
%      footnote symbol will appear for each name and footnote
%
%
% PLEASE REPORT ANY BUGS to Simon.King@ed.ac.uk
%
% Author:  Stephen Martucci  -- martucci@cdg.nj.nec.com
% Modifications: Jyri Huopaniemi -- jyri.huopaniemi@nokia.com
%                Matti Karjalainen -- matti.karjalainen@hut.fi
%                Panayiotis Georgiou -- panayiotis.georgiou@gmail.com
%                Mattias Heldner -- heldner@ling.su.se
%                Marcin W??odarczak -- wlodarczak@ling.su.se
%                Prasanta Ghosh -- prasantag@gmail.com
%                Simon King -- Simon.King@ed.ac.uk
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{INTERSPEECH2023}[2023/01/06 Official Interspeech 2023 package]

\LoadClass[a4paper]{article}

\RequirePackage{graphicx}
\RequirePackage{amssymb,amsmath,bm}
\RequirePackage{textcomp}
\RequirePackage{booktabs}
\RequirePackage[textfont=it,tableposition=top]{caption}
\RequirePackage{siunitx}
\RequirePackage{xspace}
\RequirePackage{url}
\RequirePackage{lipsum}  
\RequirePackage{tipa}
\RequirePackage{enumitem}
\RequirePackage{spconf}

% hyperref is used to ensure author names 
% do not appear in PDF metadata
\RequirePackage[pdfauthor={Author name(s) withheld},
                pdftitle={Submitted to INTERSPEECH},
                colorlinks=false,
               ]{hyperref}

% but we also tell hyperref to disable hyperlinks
\AtBeginDocument{\NoHyper}

% reasonably compact lists
\AtBeginDocument{\setlist{noitemsep,topsep=2pt,parsep=2pt,partopsep=0pt,leftmargin=1em}}

\newif\ifinterspeechfinal
\interspeechfinalfalse
\def\interspeechcameraready{\global\interspeechfinaltrue}


\newif\if@fussy
\DeclareOption{fussy}{%
  \@fussytrue
}
\DeclareOption*{\OptionNotUsed}
\ProcessOptions\relax

\if@fussy
  \fussy
\else
  \sloppy
\fi

\def\vec#1{\ensuremath{\bm{{#1}}}}
\def\mat#1{\vec{#1}}



%change default font to Times-Roman
\renewcommand{\sfdefault}{phv}
\renewcommand{\rmdefault}{ptm}
\renewcommand{\ttdefault}{pcr}

\renewcommand{\section}{\@startsection
  {section}%
  {1}%
  {}%
  {-\baselineskip}%
  {0.5\baselineskip}%
  {}}%

\renewcommand{\subsection}{\@startsection
  {subsection}%
  {2}%
  {}%
  {-\baselineskip}%
  {0.5\baselineskip}%
  {}}%

\renewcommand{\subsubsection}{\@startsection
  {subsubsection}%
  {3}%
  {}%
  {-\baselineskip}%
  {0.5\baselineskip}%
  {}}%

%% these are the A4 settings
\oddsidemargin -0.20in % -0.31in
\evensidemargin -0.20in % -0.31in
\topmargin 0truept
\headheight 0truept
\footskip 0truept % 0truept
\textheight 235truemm % 226truemm
\textwidth 170truemm % 175truemm
\voffset -41truept % -14truept
\headsep 43truept % 18truept

\twocolumn
\columnsep 10truemm % 8truemm
%% end of A4 settings

%% This is for the US 8.5 x 11 paper size
%%\oddsidemargin  -0.31in
%%\evensidemargin -0.31in
%%
%%\topmargin 0truept
%%\headheight 0truept
%%\headsep 0truept
%%\footheight 0truept % for some reason this was left commented out for is2006
%%\footskip 0truept   % for some reason this was left commented out for is2006
%%\textheight 226truemm
%%\textwidth 175truemm
%%
%%\twocolumn
%%\columnsep 8truemm
%% end of 8.5x11 bit

\pagestyle{empty}
\def\ninept{\def\baselinestretch{0.95}\let\normalsize\small\normalsize}
\def\eightpt{\def\baselinestretch{0.95}\let\normalsize\footnotesize\normalsize}
% Make 9pt the default
\ninept



% adding titlebox
\newlength\titlebox
\setlength\titlebox{5cm}
\newcommand\anonname{
	% \ifinterspeechfinal
	%      \@name
 %    \else
         Anonymous submission to INTERSPEECH 2023
    % \fi
}

\newcommand\anonaddress{
	\ifinterspeechfinal
	     \@address
    \fi
}

\newcommand\anonemail{
	\ifinterspeechfinal
	     \@email
    \fi
}


\def\maketitle{\par
 \begingroup
 \def\thefootnote{}
 \def\@makefnmark{\hbox
 to 0pt{$^{\@thefnmark}$\hss}}
 \if@twocolumn
 \twocolumn[\@maketitle]
 \else \newpage
 \global\@topnum\z@ \@maketitle \fi\@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\thefootnote{\arabic{footnote}}\gdef\@@savethanks{}%
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}


\def\@maketitle{\newpage
    {\vbox to \titlebox{
  \begin{center}
   {\large \bf \@title \par}
   \vskip 14pt {\large
     \textit{\anonname}
     \vskip 11pt
     \anonaddress}
     \vskip 3pt
     {\small\texttt{\anonemail}}
   \par\end{center}
 \par
 \thispagestyle{empty}
 \vskip 9pt}}
}

\def\title#1{\gdef\@title{\Large{#1}}}
\def\name#1{\gdef\@name{#1\\}}
\def\address#1{\gdef\@address{#1\\}}
\def\email#1{\gdef\@email{#1}}
\gdef\@title{{Title of paper}}
\gdef\@name{{\em Name of author}\\}
\gdef\@address{Address - Line 1 \\
               Address - Line 2 \\
               Address - Line 3}
\gdef\@email{email@address}



\let\@@savethanks\thanks
\def\thanks#1{\gdef\thefootnote{}\@@savethanks{#1}}
\def\sthanks#1{\gdef\thefootnote{\fnsymbol{footnote}}\@@savethanks{#1}}

\def\@sect#1#2#3#4#5#6[#7]#8{
   \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname.\hskip 0.6em}
       \begingroup \ifnum #2=1\bf\centering
          {\interlinepenalty \@M
          \large{\@svsec #8}\par}\else\ifnum #2=2\bf
          \noindent{\interlinepenalty \@M \@svsec #8\par}\else
            \it
            \ifnum #2=3
            \noindent{\interlinepenalty \@M \@svsec #8\par}
            \else\@hangfrom{\hskip\parindent}{\interlinepenalty \@M
             \@svsec #8\par}\fi\fi\fi\endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\protect\numberline{\csname the#1\endcsname} #7}
     \@tempskipa #5\relax
     \@xsect{\@tempskipa}}

\def\abstract{\begin{center}
{\bf \large Abstract\vspace{-.5em}\vspace{2pt}}
\end{center}}
\def\endabstract{\par}

\def\copyrightnotice#1{\gdef\@copyrightnotice{#1}}\let\@copyrightnotice\relax
\def\toappear#1{\gdef\@toappear{#1}}\let\@toappear\relax

%%% Strings for the preprint titlepage footer:

\newif\if@preprint\@preprintfalse
\def\ds@preprint{\@preprinttrue}
\def\ps@preprint{\let\@mkboth\@gobbletwo\def\@oddhead{}
  \def\@oddfoot{\rlap{\@toappear}\hfil\thepage\hfil
    \llap{\@copyrightnotice}\gdef\@toappear{}\gdef\@copyrightnotice{}}}

\if@preprint\ps@preprint
\else\ps@empty\flushbottom\fi

\def\thebibliography#1{\section{References}\eightpt\list
 {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

\flushbottom
%%%%% fancyheading included
\def\lhead{\@ifnextchar[{\@xlhead}{\@ylhead}}
\def\@xlhead[#1]#2{\gdef\@elhead{#1}\gdef\@olhead{#2}}
\def\@ylhead#1{\gdef\@elhead{#1}\gdef\@olhead{#1}}

\def\chead{\@ifnextchar[{\@xchead}{\@ychead}}
\def\@xchead[#1]#2{\gdef\@echead{#1}\gdef\@ochead{#2}}
\def\@ychead#1{\gdef\@echead{#1}\gdef\@ochead{#1}}

\def\rhead{\@ifnextchar[{\@xrhead}{\@yrhead}}
\def\@xrhead[#1]#2{\gdef\@erhead{#1}\gdef\@orhead{#2}}
\def\@yrhead#1{\gdef\@erhead{#1}\gdef\@orhead{#1}}

\def\lfoot{\@ifnextchar[{\@xlfoot}{\@ylfoot}}
\def\@xlfoot[#1]#2{\gdef\@elfoot{#1}\gdef\@olfoot{#2}}
\def\@ylfoot#1{\gdef\@elfoot{#1}\gdef\@olfoot{#1}}

\def\cfoot{\@ifnextchar[{\@xcfoot}{\@ycfoot}}
\def\@xcfoot[#1]#2{\gdef\@ecfoot{#1}\gdef\@ocfoot{#2}}
\def\@ycfoot#1{\gdef\@ecfoot{#1}\gdef\@ocfoot{#1}}

\def\rfoot{\@ifnextchar[{\@xrfoot}{\@yrfoot}}
\def\@xrfoot[#1]#2{\gdef\@erfoot{#1}\gdef\@orfoot{#2}}
\def\@yrfoot#1{\gdef\@erfoot{#1}\gdef\@orfoot{#1}}

\newdimen\headrulewidth
\newdimen\footrulewidth
\newdimen\plainheadrulewidth
\newdimen\plainfootrulewidth
\newdimen\headwidth
\newif\if@fancyplain
\def\fancyplain#1#2{\if@fancyplain#1\else#2\fi}

% Command to reset various things in the headers:
% a.o.  single spacing (taken from setspace.sty)
% and the catcode of ^^M (so that epsf files in the header work if a
% verbatim crosses a page boundary)
\def\fancy@reset{\restorecr
 \def\baselinestretch{1}%
 \ifx\undefined\@newbaseline% NFSS not present; 2.09 or 2e
  \ifx\@currsize\normalsize\@normalsize\else\@currsize\fi%
 \else% NFSS (2.09) present
  \@newbaseline%
 \fi}

% Initialization of the head and foot text.

\headrulewidth 0.4pt
\footrulewidth\z@
\plainheadrulewidth\z@
\plainfootrulewidth\z@

\lhead[\fancyplain{}{\sl\rightmark}]{\fancyplain{}{\sl\leftmark}}
%  i.e. empty on ``plain'' pages, \rightmark on even, \leftmark on odd pages
\chead{}
%\rhead[\fancyplain{}{\sl\leftmark}]{\fancyplain{}{\sl\rightmark}}
%  i.e. empty on ``plain'' pages, \leftmark on even, \rightmark on odd pages
\lfoot{}
\cfoot{}
\rfoot{}

% Put together a header or footer given the left, center and
% right text, fillers at left and right and a rule.
% The \lap commands put the text into an hbox of zero size,
% so overlapping text does not generate an errormessage.

\def\@fancyhead#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset\vbox{\hbox
{\rlap{\parbox[b]{\headwidth}{\raggedright#2\strut}}\hfill
\parbox[b]{\headwidth}{\centering#3\strut}\hfill
\llap{\parbox[b]{\headwidth}{\raggedleft#4\strut}}}\headrule}}#5}


\def\@fancyfoot#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset\vbox{\footrule
\hbox{\rlap{\parbox[t]{\headwidth}{\raggedright#2\strut}}\hfill
\parbox[t]{\headwidth}{\centering#3\strut}\hfill
\llap{\parbox[t]{\headwidth}{\raggedleft#4\strut}}}}}#5}

\def\headrule{{\if@fancyplain\let\headrulewidth\plainheadrulewidth\fi
\hrule\@height\headrulewidth\@width\headwidth \vskip-\headrulewidth}}

\def\footrule{{\if@fancyplain\let\footrulewidth\plainfootrulewidth\fi
\vskip-0.3\normalbaselineskip\vskip-\footrulewidth
\hrule\@width\headwidth\@height\footrulewidth\vskip0.3\normalbaselineskip}}

\def\ps@fancy{%
\@ifundefined{@chapapp}{\let\@chapapp\chaptername}{}%for amsbook
\@ifundefined{chapter}{\def\sectionmark##1{\markboth
{\uppercase{\ifnum \c@secnumdepth>\z@
 \thesection\hskip 1em\relax \fi ##1}}{}}%
\def\subsectionmark##1{\markright {\ifnum \c@secnumdepth >\@ne
 \thesubsection\hskip 1em\relax \fi ##1}}}%
{\def\chaptermark##1{\markboth {\uppercase{\ifnum \c@secnumdepth>\m@ne
 \@chapapp\ \thechapter. \ \fi ##1}}{}}
\def\sectionmark##1{\markright{\uppercase{\ifnum \c@secnumdepth >\z@
 \thesection. \ \fi ##1}}}}%
\csname ps@headings\endcsname % use \ps@headings defaults if they exist
\ps@@fancy
\gdef\ps@fancy{\@fancyplainfalse\ps@@fancy}%
\headwidth\textwidth}
\def\ps@fancyplain{\ps@fancy \let\ps@plain\ps@plain@fancy}
\def\ps@plain@fancy{\@fancyplaintrue\ps@@fancy}
\def\ps@@fancy{%
\def\@mkboth{\protect\markboth}%
\def\@oddhead{\@fancyhead\@lodd\@olhead\@ochead\@orhead\@rodd}%
\def\@oddfoot{\@fancyfoot\@lodd\@olfoot\@ocfoot\@orfoot\@rodd}%
\def\@evenhead{\@fancyhead\@rodd\@elhead\@echead\@erhead\@lodd}%
\def\@evenfoot{\@fancyfoot\@rodd\@elfoot\@ecfoot\@erfoot\@lodd}%
}
\def\@lodd{\if@reversemargin\hss\else\relax\fi}
\def\@rodd{\if@reversemargin\relax\else\hss\fi}

\let\latex@makecol\@makecol
\def\@makecol{\let\topfloat\@toplist\let\botfloat\@botlist\latex@makecol}
\def\iftopfloat#1#2{\ifx\topfloat\empty #2\else #1\fi}
\def\ifbotfloat#1#2{\ifx\botfloat\empty #2\else #1\fi}
\def\iffloatpage#1#2{\if@fcolmade #1\else #2\fi}

\def\bstctlcite{\@ifnextchar[{\@bstctlcite}{\@bstctlcite[@auxout]}}
\def\@bstctlcite[#1]#2{\@bsphack
  \@for\@citeb:=#2\do{%
    \edef\@citeb{\expandafter\@firstofone\@citeb}%
    \if@filesw\immediate\write\csname #1\endcsname{\string\citation{\@citeb}}\fi}%
  \@esphack}



==> conclusion_re.tex <==
This paper presented the design of the BSRNN-based speech enhancement and personalized speech enhancement models and the corresponding training pipeline for full-band speech signals. With the modified band-level modeling strategy and the use of MGD and MRSD training objectives, the proposed systems achieved competitive performance on various SE and PSE benchmark dataset.
As discussed in Section~\ref{sec:result}, the utilization of the SE model can significantly impair speech recognition performance. This suggests that current SE and PSE models are still suffer from model artifacts and over-suppression.
In addition, we also find that when the timbres of the target speaker and the interfering speaker are similar, the model may fail to remove the interfering speech. 
Moreover, when there is a channel mismatch between the enrollment speech and the target speech, the model may wrongly treat them as different speakers. 
We leave these issues as future works.

%In this report we describe the development of our BSRNN-based speech enhancement system. With the BSRNN model architecture and the metricgan-based adversarial training objective, the proposed system achieves SOTA performance on DNS-2020 the non-bind test set. 

==> config.tex <==


% To perform a fair comparison with existing systems under the same training and evaluation data configurations, we conduct experiments on the publicly available DNS dataset \cite{reddy2020interspeech, reddy2021interspeech}.

\subsection{Data}
\noindent\textbf{Preprocessing}: We conduct experiments on the publicly available DNS-2023 challenge dataset. 
All speech, noise, and room impulse response (RIR) data provided in the challenge are used as the training data in system development.
For the PSE task, since many of the original utterances contain more than one speaker, we first clean up the data and only keep the main speaker's speech in each utterance. Specifically, each long utterance is divided into 3-second segments first, and then the pretrained speaker embedding model is used to compute the cosine similarity between the speaker embeddings of the enrollment speech and each segment, respectively. 
The segments with cosine similarity score below 0.6 are dropped.   

\noindent\textbf{Simulation}:
During training, we performed on-the-fly data simulation to generate the 48 kHz noisy signals, where 20\% of the clean speech signals were first convolved with randomly sampled RIR filters. Note that the same RIR was applied to the enrollment and target speech in our pipeline. All the speech signals are then randomly mixed with the uniformly sampled noise with SNR range of [-5, 20] dB.
For PSE task, the interference speech signals are also added with SIR range of [-5, 20] dB. Specifically, 20\% of the training data only contained one interference speech, 50\% of the training data only contained one noise, and 30\% of the training data contained one interference speech and one noise. We used 6-second-long segments during training. The anechoic speech of the target speaker was used as the training target for dereverberation.

\begin{table*}[!ht]
    % \setlength\tabcolsep{6pt}
    \centering
    \caption{Results on DNS-2020 \textit{no\_reverb} / \textit{with\_reverb} test sets. `-16k' denotes model trained using 16 kHz data. }
    \scalebox{0.95}{
    \begin{tabular}{c|c|c|cccc|cccccccc}
    \toprule
    \hline
    \multirow{2}{*}{ID} & \multirow{2}{*}{Model} & \multirow{2}{*}{Causal} & \multicolumn{4}{c|}{\textit{no\_reverb}}  & \multicolumn{4}{c}{\textit{with\_reverb}}              \\
    & &                               & PESQ-WB   & PESQ-NB        & SI-SNR    & STOI    & PESQ-WB       & PESQ-NB & SI-SNR  & STOI \\
    \hline
    1& Noisy               & $-$       & 1.58      & 2.45 & 9.1     & 91.5     & 1.82    &2.75  & 9.0     & 86.6           \\
    2& SN-NET \cite{zheng2021interactive}              & \xmark  & 3.39      & $-$  & 19.5     & $-$      & $-$     & $-$  & $-$     & $-$             \\ 
    3& CTS-Net \cite{li2021two}            & \xmark  &2.94       & 3.42 &18.0    & 96.7     &3.02     &3.47  &15.6   &92.7            \\
    4& GaGNet  \cite{li2022glance}              & \xmark  &3.17       & 3.56 &18.9    & 97.1     &3.18     &3.57  &16.6   &93.2            \\
    5& MDNet  \cite{li2022mdnet}             & \xmark  &3.18       & 3.56 & 19.2   & 97.2     &3.24     &3.59  &16.9   &93.6             \\
    6& FRCRN \cite{zhao2022frcrn}              & \xmark  &3.23       &3.60  & 19.8    & 97.7    & $-$     & $-$ & $-$     & $-$\\
    7& DPT-FSNET \cite{dptfsnet}          & \xmark  & 3.26      & $-$  & 20.4    & 97.7     & 3.53    & $-$  &18.1    & 95.2           \\
    8& TridentSE \cite{yin2022tridentse}          & \xmark  & 3.44      & $-$  & $-$     & 97.9     & 3.50    & $-$ & $-$     & 95.2            \\
    9& MTFAA-NET \cite{zhang2022multi}          & \xmark  & \bf{3.52}      & 3.76 & $-$    & $-$        & $-$     & $-$ & $-$     & $-$              \\
    \hline
    10& BSRNN-16k             & \xmark     &3.45   &3.87   &21.1   &98.3   & \bf{3.72}  & \bf{4.03}  &19.1  &\bf{96.3} \\
    11& BSRNN                 & \xmark     &3.32   &3.79   &21.1   &98.0   & 3.54  &3.94  &18.5  &95.6  \\
    12& BSRNN-S               & \xmark     &3.42   &3.85   &21.3   &98.3   & 3.61  & 3.95 & 19.0 & 95.8\\
    13& BSRNN-S + MGD         & \xmark     &3.50   &3.85   &21.4   &98.4   & 3.63  &3.95  &19.0  &96.1 \\
    14& BSRNN-S + MRSD         & \xmark    &\bf{3.53}   &\bf{3.89}   &\bf{21.4}   &\bf{98.4}   & 3.68  &3.98  &\bf{19.2}  &\bf{96.3} \\
    % & \xmark &\bf{3.57}   &\bf{3.90}   &\bf{21.2}   &\bf{98.5}    &\bf{3.76}  &\bf{4.05}  &\bf{19.2} &\bf{96.6}   \\
    \hline
    \hline
    15& MTFAA-NET \cite{zhang2022multi}          & \cmark      & \bf{3.32}      & 3.63 & $-$     & $-$       & $-$     & $-$ & $-$     & $-$               \\
    \hline
    16& BSRNN-16k          & \cmark     &3.23       &3.73       &19.9       &97.7          &\bf{3.37}       &\bf{3.82}       &17.6 &\bf{94.8}   \\
    17& BSRNN              & \cmark     & 3.14	    &3.63	    &19.3       &  97.4        & 3.13      & 3.64      &16.8 & 93.9      \\

    18& BSRNN-S            & \cmark      & 3.26       &3.73       &20.0       &  97.6        & 3.30      & 3.77      & 17.5 & 94.5      \\
    19& BSRNN-S + MGD       & \cmark      & 3.27       &3.73       &20.1       &  97.7        & 3.33      & 3.78      & 17.4 & 94.5      \\
    
    20& BSRNN-S + MRSD      & \cmark     &\bf{3.32}   &\bf{3.77}  &\bf{20.5}  & \bf{97.8}    &\bf{3.37}  &3.80  &\bf{17.9} &94.7  \\
    \hline
    % \hline
    % pBSRNN              & 20ms          \\
    % pBSRNN-cascade      & 20ms           \\    
    % pBSRNN-cascade +MRSD      & 20ms      \\
    % % BSRNN streaming    & 20ms     &\bf{3.31}   &\bf{3.77}  &\bf{20.4}  & \bf{97.74}    &\bf{3.40}  &\bf{3.82}  &18.0 &\bf{94.79}  \\
    
    \bottomrule
    \end{tabular}
    }
    \label{tab:dns}
\end{table*}


% \begin{table}[!ht]
%     % \setlength\tabcolsep{4pt}
%     \centering
%     \caption{Performance on the DNS-2022 blind test set. PDNSMOS P.835 metrics include speech quality (SIG), background noise quality (BAK), and overall quality (OVRL).}
%     \scalebox{0.75}{
%     \begin{tabular}{c|c|ccc|ccccccccccccccccccccccc}
%     \toprule
%     \hline
%     \multirow{2}{*}{ID} &\multirow{2}{*}{Method} &\multicolumn{3}{c}{With Interference} & \multicolumn{3}{c}{Without Interference}\\
%     &                &SIG   &BAK   &OVRL  &SIG    &BAK  &OVRL \\
%     \hline
%     1& Noisy           &3.97 &1.82 &2.23 &4.22 &2.30 &2.74 \\
%     2& NSNet2\cite{braun2020data}          &3.47 &2.71 &2.44 &3.73 &4.18 &3.42 \\
%     3& DeepFilterNet2\cite{schroter2022deepfilternet2}  &3.56 &2.94 &2.68 &4.09 &4.49 &3.85 \\
%     4& TEA-PSE\cite{ju2022tea}         &3.69 &3.64 &3.16 &4.16 &4.44 &3.89 \\
%     5& TEA-PSE2\cite{ju2023tea}        &3.86 &3.83 &\bf{3.36} &4.23 &\bf{4.50} &3.98 \\
%     \hline
%     \hline
%     6& BSRNN-S         &3.76 &3.49  &3.05 &4.19 &4.51 &3.95\\
%     7& + MGD           & 3.70 &3.29 &2.93 &4.10 &4.22 &3.74 \\
%     8& + MRSD          &3.89  &3.40	 &3.10 &4.28 &\bf{4.50} &4.02 \\
%     \hline
%     9& pBSRNN-S       &3.66 &\textbf{3.91}	   &3.21     &4.17 &\bf{4.50} &3.94\\
%     10& + MRSD          &\textbf{3.90} &3.81	 &\textbf{3.37} &\textbf{4.30} &\bf{4.50} &\textbf{4.04} \\
%     \hline
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:pdns2022}
% \end{table}


\begin{table}[!ht]
    % \setlength\tabcolsep{4pt}
    \centering
    \caption{Performance on the DNS-2022 blind test set. PDNSMOS P.835 metrics include speech quality (SIG), background noise quality (BAK), and overall quality (OVRL).}
    \scalebox{0.75}{
    \begin{tabular}{c|c|ccc|ccccccccccccccccccccccc}
    \toprule
    \hline
    \multirow{2}{*}{ID} &\multirow{2}{*}{Method} &\multicolumn{3}{c}{With Interference} & \multicolumn{3}{c}{Without Interference}\\
    &                &SIG   &BAK   &OVRL  &SIG    &BAK  &OVRL \\
    \hline
    1& Noisy           &3.97 &1.82 &2.23 &4.22 &2.30 &2.74 \\
    2& NSNet2\cite{braun2020data}          &3.47 &2.71 &2.44 &3.73 &4.18 &3.42 \\
    3& DeepFilterNet2\cite{schroter2022deepfilternet2}  &3.56 &2.94 &2.68 &4.09 &4.49 &3.85 \\
    4& TEA-PSE\cite{ju2022tea}         &3.69 &3.64 &3.16 &4.16 &4.44 &3.89 \\
    5& TEA-PSE2\cite{ju2023tea}        &3.86 &3.83 &\bf{3.36} &4.23 &\bf{4.50} &3.98 \\
    \hline
    \hline
    6& BSRNN-S         &3.76 &3.49  &3.05 &4.19 &4.51 &3.95\\
    % 7& + MGD           & 3.70 &3.29 &2.93 &4.10 &4.22 &3.74 \\
    % 8& + MRSD          &3.89  &3.40	 &3.10 &4.28 &\bf{4.50} &4.02 \\
    % \hline
    7& pBSRNN-S       &3.66 &\textbf{3.91}	   &3.21     &4.17 &\bf{4.50} &3.94\\
    8& + MRSD          &\textbf{3.90} &3.81	 &\textbf{3.37} &\textbf{4.30} &\bf{4.50} &\textbf{4.04} \\
    \hline
    \bottomrule
    \end{tabular}
    }
    \label{tab:pdns2022}
\end{table}

\begin{table}[!ht]
    \setlength\tabcolsep{3pt}
    \centering
    \caption{Results on the blind test set of DNS-2023}
    \scalebox{0.8}{
    \begin{tabular}{c|ccc|ccccccccccccccccccccccc}
    \toprule
    \hline
    \multirow{2}{*}{Method} &\multicolumn{3}{c}{Headset track} & \multicolumn{3}{c}{Speakerphone track}\\
                    &OVRL   &WACC   &SCORE  &OVRL   &WACC   &SCORE \\
    \hline
    Noisy           &1.22 &0.843 &0.449 &1.24 &0.857 &0.459 \\
    Baseline        &2.34 &0.687 &0.511 &2.38 &0.727 &0.537 \\
    pBSRNN-S + MRSD  &2.65 &0.724 &0.568 &2.66 &0.724  &0.570 \\
    \hline
    \bottomrule
    \end{tabular}
    }
    \label{tab:pdns2023}
\end{table}


\subsection{Model Configuration}

\noindent\textbf{Band-spilt Scheme}: We split the frequency band below 4 kHz by a 200 Hz bandwidth, the frequency band between 4 kHz and 8 kHz by a 500 Hz bandwidth, and the frequency band above 8 kHz by a 2 kHz bandwidth. This results in 33 subbands.

\noindent\textbf{Hyperparameters}: 
We set the window and hop sizes of short-time Fourier transform (STFT) to 20 ms and 10 ms for 48kHz model, and 32 ms and 8 ms for 16 kHz model.
Hanning window is applied as the analysis window.  
We set the feature dimension $N$ in the BSRNN model to 96 for 48 kHz model and 128 for 16 kHz model, and we use 6 band and sequence modeling modules. We set the hidden unit of the LSTM layers to $2N=192$, the hidden size in the mask estimation MLPs to be $4N=384$, and use the hyperbolic tangent function as the nonlinear activation function in the MLP. We use a gated linear unit (GLU) \cite{dauphin2017language} for the output layer of the MLP when generating the contextual complex-valued masks. We use layer normalization \cite{ba2016layer} for offline configuration and batch normalization \cite{ioffe2015batch} for online configuration throughout the model. The computational complexity of the online pBSRNN model is around 14.7G multiply-accumulate operations (MACs) per second and the real-time factor (RTF) is around 0.42 with ONNX-runtime implementation on Intel i5 CPU @2.50GHz.

\noindent\textbf{Speaker Embedding Model}: The pretrained speaker embedding model \cite{chen2022sjtu}\footnote{\url{https://github.com/wenet-e2e/wespeaker/blob/master/docs/pretrained.md}} constructed using the VoxCeleb \cite{chung2018voxceleb2} dataset is used in our model.

\subsection{Training Pipeline}
For non-personlized speech enhancement, we first train the BSRNN model (without speaker enrollment module) from scratch using the MR loss with initial learning rate of $1e^{-3}$ for 400k iteration. Then, we finetune the model with the MGD and MRSD training objectives for another 100k iterations.
The training of PSE model is similar to the no-personlized model, and the only difference is that the PSE model uses the parameters of the pretrained non-personlized model as initialization.
All the models are optimized using Adam optimizer. 
The learning rate is decayed by 0.98 for every 20k iterations, and gradient clipping by a maximum gradient norm of 5 is applied.
Early stopping is applied when the best validation is not found in 20k consecutive iterations.
8 Nvidia Tesla P40 GPUs were used with a batch size of 12 per GPU. 



==> data.tex <==
We followed the same data preprocessing setup for both the headset and speaker phone tracks in the DNS 2023 challenge. 
All speech, noise, and room impulse response (RIR) data provided in the challenge were used as the training data in system development.

\subsection{Data Preprocessing}
Since a large number of the original “readspeech” long utterances contain more than one speaker, we first cleaned up the data and only kept the main speaker's speech in each utterance. Specifically, each long utterance was divided into several 3 second segments first, and then a pretrained speaker verification model was used to compute the cosine similarity between the speaker embeddings of the enrollment speech and each segment, respectively. 
The segments whose similarities are below 0.6 were dropped.   

\subsection{Data Simulation}
During training, we performed on-the-fly data simulation to generate the 48 kHz noisy signals, where 20\% of the clean speech signals were first convolved with randomly sampled RIR filters. Note that the same RIR was applied to the enrollment and target speech in our pipeline. The echoic signals were then randomly mixed with the uniformly sampled noise and interference speech signals with SNR range of [-5, 20] dB and SIR range of [-5, 20] dB. During training, 20\% of the training data only contained one interference speech, 50\% of the training data only contained one noise, and 30\% of the training data contained one interference speech and one noise. We used 6-second-long segments during training. The anechoic speech of the target speaker was used as the training target for dereverberation. 



==> intro.tex <==
% 语音增强有广泛的应用
Speech enhancement (SE) is an important task in speech communication that aims to improve the subjective and objective quality of speech signals. 
Such improvements can not only be helpful for human listeners to better understand the contents but also be beneficial for machine listeners to generate more accurate transcriptions. 
Over the past few years, the performance of deep neural network (DNN)-based speech enhancement systems has been considerably advanced thanks to the development of novel model architectures \cite{tan2019learning, xu2014regression, dccrn, fullsubnet, BSRNN, demucs, li2021two, pascual2017segan, li2022glance, wang2021tstnn, kim2021se}, training objectives \cite{remixit, xia2020weighted, fu2019metricgan}, and world-wide competitions with large-scale training data and realistic evaluation configurations \cite{reddy2021icassp}. 
Recently, with the increasing demand for high-fidelity (Hi-Fi) speech in online conferencing systems and high-definition live streaming, speech enhancement models have also been expanded to deal with super wide-band (24 kHz) and full-band (48 kHz) speech signals \cite{S-DCCRN, zhang2022multi, dptfsnet}.
Moreover, since conventional SE models cannot suppress the speech of interfering speakers, personalized SE (PSE) models have also been proposed \cite{wang2018voicefilter, wang2020voicefilter, giri2021personalized, ju2022tea, ju2023tea} to extract the voice of the target speaker from background noise and other interfering speech sources using the enrolled target speaker information.

Although previous SE and PSE models can largely improve the quality of the desired speech signals, the performance of these models on full-band signals is restricted by the following two aspects.
First, in real-time speech communication, different devices have various effective sample rates and frequency responses. 
Some devices can precisely capture high-frequency ($>$16 kHz) information of the speech signal, while others may introduce significant distortion in the high-frequency range. 
Such unpredictable device-dependent distortion on high-frequency components can degrade the performance of full-band speech enhancement.
Second, the conventional training objectives of SE models, such as signal-to-noise ratio (SNR) and frequency-domain mean square error (MSE), are not closely related to human auditory perception and other objective perceptual metrics, which can lead to sub-optimal SE performance. 

\begin{figure*}[!htb]
	\centering
	\includegraphics[width=1\linewidth]{Figures/BSRNN-pse-L.pdf}
    \caption{The architecture of the BSRNN framework for full-band PSE task. (A) The design of the band split module. (B) The design of the sequence and band modeling module. (C) The design of the estimation module. (D) The design of the speaker enrollment module.}
\label{fig:BSRNN}
\end{figure*}

In this paper, we attempt to address the aforementioned issues by extending the recently proposed source separation model, the \textit{band-split RNN (BSRNN)} \cite{BSRNN}, which has achieved state-of-the-art (SOTA) performance on a publicly available music separation dataset, to the tasks of full-band SE and PSE.
In the modified BSRNN, the spectrogram of the input signal is first split into a set of frequency bands and then transformed into a series of subband features with band-specific fully connected (FC) layers. 
For full-band SE and PSE tasks, we perform bi-directional band-level modeling for subbands below 16 kHz and uni-directional modeling for subbands above 16 kHz to mitigate the effect of high-frequency distortion introduced by the devices.
% Two band-specific multilayer perceptrons (MLPs) are then used to estimate the complex-valued time-frequency (T-F) mask and the complex-valued residual spectrogram of the target speech. The final output spectrogram is obtained by adding the masked and the residual spectrogram.
% Then, we perform bi-directional band-level modeling for subbands below 16 kHz and uni-directional modeling for subbands above 16 kHz.
For PSE task, an additional speaker enrollment module is added to BSRNN to make use of the target speaker information.
% \sout{A complex-valued time-frequency (T-F) mask is then calculated by transforming the output of the last RNN layer with band-specific multilayer perceptrons (MLPs).}
% To mitigate the effect of high-frequency distortion introduced by the devices, for full-band SE and PSE tasks, we perform bi-directional band-level modeling for subbands below 16 kHz and uni-directional modeling for subbands above 16 kHz.
In addition, we use a modified MetricGAN-based training objective \cite{fu2019metricgan, fu2021metricgan+} to directly optimize the model towards the widely-used perceptual evaluation of speech quality (PESQ) score.
Moreover, to improve the human auditory perceptual quality, we also optimize the model with a multi-resolution spectrogram discriminator (MRSD) \cite{jang2021univnet}.
Experimental results show that our BSRNN system outperforms various top-ranking benchmark systems in SE and achieves SOTA results on the DNS-2020 non-blind test set in both offline and online scenarios.
In addition, the proposed system achieves competitive performance on PSE and ranks 3rd in both the headset track and speaker phone track in the 5th deep noise suppression (DNS-2023) challenge.

The rest of the paper is organized as follows. Section~\ref{sec:model} introduces the proposed BSRNN architecture. Section~\ref{sec:obj} presents the training objectives. Section~\ref{sec:config} provides the configurations for data simulation and training. Section~\ref{sec:result} presents the experiment results and analysis.  Section~\ref{sec:conclusion} concludes the paper.


% we utilize a MetricGAN-based discriminator (MGD) and a multi-resolution spectrogram-based discriminator (MRSD) in system training to improve non-differentiable perceptual quality metrics such as perceptual evaluation of speech quality (PESQ) and PDNSMOS. 


% 作为 technical report， 感觉这个地方意义不大
% Among all the previous SE frameworks, the recently proposed multi-scale temporal frequency convolutional network with axial self-attention network (MTFAA-Net), has shown the most competitive performance and ranked 1st in the latest ICASSP 2022 DNS challenge (DNS-4th) \cite{dns4}. The MTFAA-net utilizes a set of techniques including two-stage mask, ERB band merging \cite{}, convolution neural network (CNN) based frequency downsampling and upsampling, and dual-path self-attention model architecture to boost the performance of the system, which result in a relatively complicated framework for reproduction.     

% Existing systems for speech enhancement, including the participants of the deep noise suppression (DNS) challenges, are mostly directly designed and evaluated for this specific task. This report attempts to perform a ``reversed process'': we adopt our recently proposed model for music separation, i.e. the \textit{band-split RNN (BSRNN)} model \cite{BSRNN}, which achieved state-of-the-art (SOTA) performance on a public available music separation dataset, to the task of speech enhancement. Given that the background music can be viewed as a (more) complicated interference signal that distorts the vocal sound, the process of extracting the vocal sound from a piece of music can be viewed as a generalized speech enhancement process. 
% Moreover, to directly optimize the model towards widely-used evaluation metrics such as perceptual evaluation of speech quality (PESQ), we use a modified MetricGAN-based training objective \cite{fu2019metricgan, fu2021metricgan+} to further improve the overall performance of the BSRNN model. We train the model on the training data of Interspeech 2021 DNS challenge \cite{reddy2021interspeech} and evaluate on the DNS-2020 \textit{no\_reverb} and
% \textit{with\_reverb} test sets, and the results show that the BSRNN system outperforms various top-ranking systems and achieves state-of-the-art results (SOTA) on various evaluation metrics in both offline and online configurations. This proves that the BSRNN architecture has the potential to become a general design paradigm for various speech processing tasks. 



%The performance improvement of our system comes from the adoption of the BSRNN model architecture and the MetricGAN-based adversarial training objective \cite{fu2021metricgan+}.

% The remainder of the report describes the design of the BSRNN model, the MetricGAN-based training objective, the experiment configurations, and the results and discussions.


% 1) SE is important-> High frequency SE and PSE
% 2) Challenge: unstable high frequency response: cascade 
% 3) Loss Function 
% 4) PSE


==> model.tex <==
The BSRNN model depicted in Figure~\ref{fig:BSRNN} is a frequency-domain model consists of a \textit{band split module}, a \textit{band and sequence modeling module}, a \textit{mask estimation module} and an additional \textit{speaker enrollment module} for PSE.
As shown in Figure~\ref{fig:BSRNN} (A), the band split module explicitly splits the complex-valued spectrogram of the noisy input $\vec{X}$ into a set of non-overlapped frequency bands $\{\vec{B}_i\}_{i=1}^{K}$ and generates a series of subband features $\{\vec{Z}_i\}_{i=1}^{K}$ with band-specific FC layers.
The band and sequence modeling module utilizes residual long short-term memory networks (LSTMs) to perform interleaved band-level and sequence-level modeling on the subband features $\vec{Z}$. 

As discussed in Section~\ref{sec:intro}, different recording devices can introduce unpredictable distortions and information lost in high-frequency components (normally $>$16 kHz) due to different frequency responses. For example, the frequency components above 16 kHz are missing in the spectrogram shown in Figure~\ref{fig:BSRNN} (A). 
Hence, the bi-directional intra-band modeling used in original BSRNN model \cite{BSRNN} can be sub-optimal, as it can propagate high-frequency distortions to lower frequencies and thereby compromise the overall enhancement performance. To attenuate the effects of the high-frequency distortions in full-band enhancement, we split the subband features $\hat{\vec{Z}}$ to  $\hat{\vec{Z}_1}$ and $\hat{\vec{Z}_2}$, where $\hat{\vec{Z}_1}$ contains the subband features below 16 kHz and $\hat{\vec{Z}_2}$ contains subbands above 16 kHz. Then we perform bi-directional band-level modeling on  $\hat{\vec{Z}_1}$ and uni-directional modeling on $\hat{\vec{Z}_2}$ as follows: 
\begin{align}
    \vec{Q}_1, (\vec{h}, \vec{c}) = \text{BLSTM}(\hat{\vec{Z}}_1); \ \ \  \vec{Q}_2 = \text{LSTM}(\hat{\vec{Z}}_2, (\vec{h}, \vec{c}))
\end{align}
where $\vec{h}$ and $\vec{c}$ are the hidden and cell state of the low-to-high direction obtained from the band-level modeling of $\hat{\vec{Z}}_2$. In the rest of the paper, we will use \textit{BSRNN-S} to denote the BSRNN model with split band-level modeling.

After the band and sequence modeling module, the estimation module uses band-specific MLPs to predict the complex-value T-F mask $\vec{M} \in \mathbb{C}^{F \times T}$. 
To attenuate the artifacts introduced by the T-F mask, an additional MLP is used to directly predict the complex-valued residual spectrogram $\vec{R}\in \mathbb{C}^{F \times T}$ of the target speech. The final output can be obtained as:
\begin{align}
    \bar{\vec{S}} =  \vec{M} \odot \vec{X} + \vec{R}
\end{align}
where $\odot$ denotes the complex-valued element-wise multiplication and $ \bar{\vec{S}}$ represents the output spectrogram.

To remove interfering speech in PSE task, a speaker enrollment module is used to extract the target speaker information from the enrollment speech. 
Specifically, the enrollment speech is a pre-recorded 5 to 10 seconds clean or noisy speech segment from the target speaker, which is used to compute the speaker embedding $e\in\mathbb{R}^{F}$. In the proposed model, a pretrained speaker embedding model based on ResNet34 with freezed model parameters is used to compute the speaker embedding $e$.
The speaker embedding is then transformed into band-level features by 1-D convolutional layers with $K$ output channels using \textit{Tanh} nonlinear activation and repeated along the temporal dimension to form the speaker representation $\mathbf{E}\in\mathbb{R}^{K\times T \times N}$. 
The speaker representation $\mathbf{E}$ and the subband feature $\mathbf{Z}$ are concatenated along the feature dimension and then used to perform interleaved band-level and sequence-level modeling. In the rest of the paper, we will use pBSRNN to denote the personalized BSRNN model.
% The band-specific mask estimation modules estimates the complex-valued time-frequency (T-F) masks $\{\vec{M}\}_{i=1}^{K}$ by transforming each output of the last residual RNN layer $\{\vec{Q}\}_{i=1}^{K}$ with a multilayer perceptron (MLP).

% \subsection{Modified Band-Split RNN}
% To achieve high fidelity full-band SE and PSE, we modified the original BSRNN model from three aspects as shown in Figure~\ref{fig:BSRNN}.
% First, an enrollment module was used to extract the target speaker information from the speaker embedding $\mathbf{e}\in\mathbb{R}^{F}$ of the enrollment speech. 
% The speaker embedding was first transformed into band-level features by 1-D convolutional layers with $K$ output channels using \textit{Tanh} nonlinear activation and then repeated along the time dimension to form the speaker representation $\mathbf{E}\in\mathbb{R}^{K\times T \times N}$. 
% The speaker representation $\mathbf{E}$ and the subband feature $\mathbf{Z}$ were concatenated along the feature dimension and then used to perform interleaved band-level and sequence-level modeling.

% Second, since the high-frequency subband features can be unstable due to the different frequency responses of various microphones, we applied uni-directional and bi-directional band-level modeling to subbands above 8 kHz and subbands below 8 kHz, respectively, to mitigate the effects of unstable high-frequency components.
% In addition, to attenuate the distortion introduced by the time-frequency (T-F) mask, an additional MLP model was also added in the estimation module to directly estimate the complex spectrogram of the target speech. The final output can be obtained as follows:
% \begin{align}
%     \bar{\vec{S}} =  \vec{M} \odot \vec{X} + \vec{R}
% \end{align}
% where $\odot$ denotes the complex-valued element-wise product, $\vec{X}$, $\bar{\vec{S}}$ and $\vec{R}$ represent the input, the output, and the MLP-estimated spectrogram respectively. $\vec{M}$ is the predicted T-F mask.

  
% First, 
% 1) speaker enrollment
% 2) frequency divide
% 3) regression frequency estimation 
% in our system


% The BSRNN model, first proposed in \cite{BSRNN} and depicted in Figure~\ref{fig:BSRNN}, is a frequency-domain model consists of a \textit{band split module}, a \textit{band and sequence modeling module} and a \textit{mask estimation module}.
% The band split module explicitly splits the complex-valued spectrogram of the noisy input $\vec{X}$ into a set of non-overlapped frequency bands $\{\vec{B}_i\}_{i=1}^{K}$ and generates a series of subband features $\{\vec{Z}_i\}_{i=1}^{K}$ with band-specific fully connected (FC) layers.
% The band and sequence modeling module utilizes two residual recurrent neural networks (RNNs) to perform interleaved band-level and sequence-level modeling on the subband features $\vec{Z}_i$. 
% The band-specific mask estimation modules estimates the complex-valued time-frequency (T-F) masks $\{\vec{M}\}_{i=1}^{K}$ by transforming each output of the last residual RNN layer $\{\vec{Q}\}_{i=1}^{K}$ with a multilayer perceptron (MLP). Moreover, we use a contextual mask similar to \cite{deepfilternet} to incorporate the neighbouring T-F bins into the final output:
% \begin{align}
%     \bar{\vec{S}}_t = \sum_{t=-1}^{T=1} \vec{M}_t \odot \vec{X}_t
% \end{align}
% where $\odot$ denotes the complex-valued element-wise product, $\vec{X}_t$ and $\bar{\vec{S}}_t$ represent the $t$-th frames of the input and the enhanced spectrograms, respectively.

==> objective.tex <==
The training objective of our model contains three parts. 

% \subsection{Multi-resolution Frequency Loss}
\noindent\textbf{Multi-resolution Frequency Loss}:
The first part is a multi-resolution (MR) frequency-domain loss $\mathcal{L}_{MR}$ designed by combining the power-compressed amplitude mean average error (MAE) loss and the complex-valued MAE loss with STFT windows ranging from 10 ms to 40 ms: 
\begin{align}
    \mathcal{L}_{MR} = \frac{1}{I}\sum_{i} \left( \Arrowvert|\vec{S}_i|^{p} - |\bar{\vec{S}}_{i}|^{p}\Arrowvert_1 + \Arrowvert\vec{S}_{i} - \bar{\vec{S}}_{i}\Arrowvert_1\right) 
\end{align}
where ${\vec{S}}_{i}$ and ${\bar{\vec{S}}}_{i}$ are the complex-valued spectrograms with window sizes in \{10, 20, 30, 40\} ms of the target and estimated speech, and $p$ is set to 0.3. 


% \subsection{MetricGAN}

\noindent\textbf{MetricGAN}: To directly improve the system performance on the PESQ score, adversarial training based on MetricGAN (MGD) \cite{fu2019metricgan, fu2021metricgan+} is adopted.
The generator of MGD is the BSRNN model and the discriminator in MGD $D(\cdot)$ attempts to predict the normalized PESQ score:
\begin{align}
    Q_{\text{PESQ}}(\bar{\vec{S}}, {\vec{S}}) = \frac{\text{PESQ}(\bar{\vec{S}}, \vec{S}) + 0.5}{5} 
\end{align}
Note that the wide-band PESQ score is used in all experiments. Two least-square GAN (LSGAN) \cite{mao2017least} style training objectives are then designed for the generator and discriminator:
\begin{align}
    \mathcal{L}_{d} &= (1 - D({\vec{S}}, \vec{S}))^{2} + (Q_{\text{PESQ}}(\bar{\vec{S}}, \vec{S}) - D(\bar{\vec{S}}, \vec{S}))^{2} \\ \nonumber 
        &+ (Q_{\text{PESQ}}({\vec{X}}, {\vec{S}} ) - D({\vec{X}}, {\vec{S}}))^{2} \\
    \mathcal{L}_{g} &= (1 - D(\bar{\vec{S}}, \vec{S}))^{2} + 0.5 \cdot \mathcal{L}_{MR}
\end{align}
where $\mathcal{L}_{g}, \mathcal{L}_{d}$ denote the generator loss and the discriminator loss, respectively. Note that the discriminator loss contains three signal pairs from noisy input, clean target and estimated target to stabilize the training process.

% \subsection{Multi-resolution Spectrogram Discriminator}
\noindent\textbf{Multi-resolution Spectrogram Discriminator}:
Following \cite{jang2021univnet}, a multi-resolution spectrogram discriminator (MRSD) is used to improve the perceptual quality metric score of the model: 
\begin{align}
    &\mathcal{L}_{D} = \frac{1}{K} \sum_{k} \left( (1 - D_{k}(\vec{S}))^{2} +D_{k}(\bar{\vec{S}})^{2} \right)  \\
    &\mathcal{L}_{G} = \frac{1}{K} \sum_{k} (1 - D_{k}(\bar{\vec{S}}))^{2}  + \mathcal{L}_{\text{MR}} + \mathcal{L}_{\text{MMEL}}
\end{align}
where $\mathcal{L}_{D}, \mathcal{L}_{G}$ denote the generator and discriminator loss, respectively, and $k$ is the STFT window length index from [2, 4, 8, 16, 32, 64] ms. $\mathcal{L}_{\text{MMEL}}$ is the multi-frequency mel-spectrogram MSE loss.



\iffalse
The training objective for our model contains two parts. The first part is a frequency-domain loss designed by combining the power-compressed amplitude mean average error (MAE) loss $\mathcal{L}_{p}$ and the complex-valued MAE loss $\mathcal{L}_{s}$:
\begin{align}
    &\mathcal{L}_{p} =  |||\vec{S}|^{p} - |\bar{\vec{S}}|^{p}||_1 \\
    &\mathcal{L}_{s} = ||\vec{S} - \bar{\vec{S}}||_1
\end{align}
where ${\vec{S}}$ denotes the complex-valued spectrogram of the target signal, and $p$ is set to 0.3. The second part is a modified MetricGAN-based objective particularly designed for the PESQ score.
%The proposed BSRNN is optimized  with the power-compressed amplitude Mean Average Error (MAE) loss $\mathcal{L}_{p}$ and the complex spectrogram MAE loss $\mathcal{L}_{s}$.
%\begin{align}
%    &\mathcal{L}_{p} =  ||\vec{S}|^{p} - |\bar{\vec{S}}|^{p}|_1 \\
%    &\mathcal{L}_{s} = |\vec{S} - \bar{\vec{S}}|_1
%\end{align}
%To directly improve the system performance on the perceptual evaluation of speech quality (PESQ) score, adversarial training based on MetricGAN \cite{fu2019metricgan, fu2021metricgan+} is adopted. 
Following \cite{fu2021metricgan+}, the modified MetricGAN pipeline also contains a generator and a discriminator, where the generator is the BSRNN model to generate the estimated target spectrogram $\bar{\vec{S}}$ and the discriminator $D(\cdot)$ attempts to estimate the normalized PESQ score of a pair of spectrograms:
\begin{align}
    Q_{\text{PESQ}}(\bar{\vec{S}}, {\vec{S}}) = \frac{\text{PESQ}(\bar{\vec{S}}, \vec{S}) + 0.5}{5} 
\end{align}
where we use wide-band PESQ score in all experiments. Two least-square GAN (LSGAN) \cite{mao2017least} style training objectives are then designed for the generator and discriminator, respectively:
\begin{align}
    &\mathcal{L}_{g} = (1 - D(\bar{\vec{S}}, \vec{S}))^{2} \\
    &\mathcal{L}_{d} = (1 - D({\vec{S}}, \vec{S}))^{2} + (Q_{\text{PESQ}}(\bar{\vec{S}}, \vec{S}) - D(\bar{\vec{S}}, \vec{S}))^{2} \\ \nonumber 
    &+ (Q_{\text{PESQ}}({\vec{X}}, {\vec{S}} ) - D({\vec{X}}, {\vec{S}}))^{2}
\end{align}
where $\mathcal{L}_{g}, \mathcal{L}_{d}$ denote the generator loss and the discriminator loss, respectively. Note that the discriminator loss contains three signals pairs from noisy input, clean target and estimated target in order to stabilize the training process. The final loss for the BSRNN model (i.e. the generator) is then formulated as follows:
\begin{align}
    \mathcal{L}_{obj} = \lambda_{1}\cdot\mathcal{L}_{p} +  \lambda_{2}\cdot\mathcal{L}_{s} + \lambda_{3}\cdot\mathcal{L}_{g}
\end{align}
where $\lambda_{1}, \lambda_{2}, \lambda_{3}$ are the weights of the corresponding components, and we set $\lambda_{1}=0.5$, $\lambda_{2}=0.5$, 
and $\lambda_{3}=1$.


\begin{align}
    Q_{\text{PESQ}}(\vec{S}, \bar{\vec{S}}) = \frac{\text{PESQ}(\vec{S}, \bar{\vec{S}}) + 0.5}{5} 
\end{align}
Note that we used wide-band PESQ in all the experience.
The final loss is formulated as follows:
\begin{align}
    \mathcal{L}_{obj} = \lambda_{1}*\mathcal{L}_{p} +  \lambda_{2}*\mathcal{L}_{s} + \lambda_{3}*\mathcal{L}_{g}
\end{align}
where $\lambda_{1}, \lambda_{2}, \lambda_{3}$ are the weights of the corresponding losses, we set  $\lambda_{1}=0.5, \lambda_{2}=0.5, \lambda_{3}=1$ in all our experiments.
\fi

==> pipeline.tex <==
The training objective for our model contains three parts.
A multi-resolution (MR) frequency-domain loss $\mathcal{L}_{MR}$ was designed by combining the power-compressed amplitude mean average error (MAE) loss and the complex-valued MAE loss with STFT with windows from 10 ms to 40 ms: 
\begin{align}
    \mathcal{L}_{MR} = \frac{1}{I}\sum_{i} \left( \Arrowvert|\vec{S}_i|^{p} - |\bar{\vec{S}}_{i}^{p}|\Arrowvert_1 + \Arrowvert\vec{S}_{i} - \bar{\vec{S}}_{i}\Arrowvert_1\right) 
\end{align}
where ${\vec{S}}_{i}$ and ${\bar{\vec{S}}}_{i}$ are the complex-valued spectrograms with window sizes in \{10, 20, 30, 40\} ms of the target and estimated speech, and $p$ is set to 0.3. 


\subsection{MetricGAN}
Following \cite{fu2021metricgan+}, the modified MetricGAN pipeline also contains a generator and a discriminator, where the generator is the BSRNN model to generate the estimated target spectrogram $\bar{\vec{S}}$ and the discriminator $D(\cdot)$ attempts to estimate the normalized PESQ score of a pair of spectrograms:
\begin{align}
    Q_{\text{PESQ}}(\bar{\vec{S}}, {\vec{S}}) = \frac{\text{PESQ}(\bar{\vec{S}}, \vec{S}) + 0.5}{5} 
\end{align}
where we use wide-band PESQ score in all experiments. Two least-square GAN (LSGAN) \cite{mao2017least} style training objectives are then designed for the generator and discriminator, respectively:
\begin{align}
    &\mathcal{L}_{g} = (1 - D(\bar{\vec{S}}, \vec{S}))^{2} \\
    &\mathcal{L}_{d} = (1 - D({\vec{S}}, \vec{S}))^{2} + (Q_{\text{PESQ}}(\bar{\vec{S}}, \vec{S}) - D(\bar{\vec{S}}, \vec{S}))^{2} \\ \nonumber 
    &+ (Q_{\text{PESQ}}({\vec{X}}, {\vec{S}} ) - D({\vec{X}}, {\vec{S}}))^{2}
\end{align}
where $\mathcal{L}_{g}, \mathcal{L}_{d}$ denote the generator loss and the discriminator loss, respectively. Note that the discriminator loss contains three signals pairs from noisy input, clean target and estimated target in order to stabilize the training process. The final loss for the BSRNN model (i.e. the generator) is then formulated as follows:
\begin{align}
    \mathcal{L}_{obj} = \lambda_{1}\cdot\mathcal{L}_{p} +  \lambda_{2}\cdot\mathcal{L}_{s} + \lambda_{3}\cdot\mathcal{L}_{g}
\end{align}
where $\lambda_{1}, \lambda_{2}, \lambda_{3}$ are the weights of the corresponding components, and we set $\lambda_{1}=0.5$, $\lambda_{2}=0.5$, 
and $\lambda_{3}=1$.

\subsection{Multi-resolution Spectrogram Discriminator}
Following \cite{jang2021univnet}, a multi-resolution spectrogram discriminator (MRSD) is used to improve the perceptual quality metric score of the model
\begin{align}
    &\mathcal{L}_{D} = \frac{1}{K} \sum_{k} \left( (1 - D_{k}(\vec{S}))^{2} +D_{k}(\bar{\vec{S}})^{2} \right)  \\
    &\mathcal{L}_{G} = \frac{1}{K} \sum_{k} (1 - D_{k}(\bar{\vec{S}}))^{2}  + \mathcal{L}_{MR} + \mathcal{L}_{MMEL}
\end{align}
where $\mathcal{L}_{D}, \mathcal{L}_{G}$ denote the generator and discriminator loss, respectively, and $k$ is the STFT window length index from [2, 4, 8, 16, 32, 64] ms. $\mathcal{L}_{MMEL}$ is the multi-frequency mel-spectrogram MSE loss.



\iffalse
The training objective for our model contains two parts. The first part is a frequency-domain loss designed by combining the power-compressed amplitude mean average error (MAE) loss $\mathcal{L}_{p}$ and the complex-valued MAE loss $\mathcal{L}_{s}$:
\begin{align}
    &\mathcal{L}_{p} =  |||\vec{S}|^{p} - |\bar{\vec{S}}|^{p}||_1 \\
    &\mathcal{L}_{s} = ||\vec{S} - \bar{\vec{S}}||_1
\end{align}
where ${\vec{S}}$ denotes the complex-valued spectrogram of the target signal, and $p$ is set to 0.3. The second part is a modified MetricGAN-based objective particularly designed for the PESQ score.
%The proposed BSRNN is optimized  with the power-compressed amplitude Mean Average Error (MAE) loss $\mathcal{L}_{p}$ and the complex spectrogram MAE loss $\mathcal{L}_{s}$.
%\begin{align}
%    &\mathcal{L}_{p} =  ||\vec{S}|^{p} - |\bar{\vec{S}}|^{p}|_1 \\
%    &\mathcal{L}_{s} = |\vec{S} - \bar{\vec{S}}|_1
%\end{align}
%To directly improve the system performance on the perceptual evaluation of speech quality (PESQ) score, adversarial training based on MetricGAN \cite{fu2019metricgan, fu2021metricgan+} is adopted. 
Following \cite{fu2021metricgan+}, the modified MetricGAN pipeline also contains a generator and a discriminator, where the generator is the BSRNN model to generate the estimated target spectrogram $\bar{\vec{S}}$ and the discriminator $D(\cdot)$ attempts to estimate the normalized PESQ score of a pair of spectrograms:
\begin{align}
    Q_{\text{PESQ}}(\bar{\vec{S}}, {\vec{S}}) = \frac{\text{PESQ}(\bar{\vec{S}}, \vec{S}) + 0.5}{5} 
\end{align}
where we use wide-band PESQ score in all experiments. Two least-square GAN (LSGAN) \cite{mao2017least} style training objectives are then designed for the generator and discriminator, respectively:
\begin{align}
    &\mathcal{L}_{g} = (1 - D(\bar{\vec{S}}, \vec{S}))^{2} \\
    &\mathcal{L}_{d} = (1 - D({\vec{S}}, \vec{S}))^{2} + (Q_{\text{PESQ}}(\bar{\vec{S}}, \vec{S}) - D(\bar{\vec{S}}, \vec{S}))^{2} \\ \nonumber 
    &+ (Q_{\text{PESQ}}({\vec{X}}, {\vec{S}} ) - D({\vec{X}}, {\vec{S}}))^{2}
\end{align}
where $\mathcal{L}_{g}, \mathcal{L}_{d}$ denote the generator loss and the discriminator loss, respectively. Note that the discriminator loss contains three signals pairs from noisy input, clean target and estimated target in order to stabilize the training process. The final loss for the BSRNN model (i.e. the generator) is then formulated as follows:
\begin{align}
    \mathcal{L}_{obj} = \lambda_{1}\cdot\mathcal{L}_{p} +  \lambda_{2}\cdot\mathcal{L}_{s} + \lambda_{3}\cdot\mathcal{L}_{g}
\end{align}
where $\lambda_{1}, \lambda_{2}, \lambda_{3}$ are the weights of the corresponding components, and we set $\lambda_{1}=0.5$, $\lambda_{2}=0.5$, 
and $\lambda_{3}=1$.


\begin{align}
    Q_{\text{PESQ}}(\vec{S}, \bar{\vec{S}}) = \frac{\text{PESQ}(\vec{S}, \bar{\vec{S}}) + 0.5}{5} 
\end{align}
Note that we used wide-band PESQ in all the experience.
The final loss is formulated as follows:
\begin{align}
    \mathcal{L}_{obj} = \lambda_{1}*\mathcal{L}_{p} +  \lambda_{2}*\mathcal{L}_{s} + \lambda_{3}*\mathcal{L}_{g}
\end{align}
where $\lambda_{1}, \lambda_{2}, \lambda_{3}$ are the weights of the corresponding losses, we set  $\lambda_{1}=0.5, \lambda_{2}=0.5, \lambda_{3}=1$ in all our experiments.
\fi

==> result.tex <==
\subsection{Non-personalized speech-enhancement}
Table~\ref{tab:dns} compares the performance between the proposed non-personalized SE BSRNN models and several top-ranking benchmark models on the non-blind test of DNS-2020 challenge.
It can be observed that: 
1) Compared with models trained using wide-band (16 kHz) data, the performance of models trained on full-band data with bi-directional band-level modeling degrades significantly (ID 10 v.s. 11, ID 16 v.s. 17), which supports the claim that the high-frequency distortion can degrade the full-band enhancement performance;
2) Using bi-directional and uni-directional band-level modeling on low-frequency and high-frequency subbands separately can improve the performance of full-band SE models (ID 11 v.s. 12, ID 17 v.s. 18);
3) The use of MGD and MRSD training objectives can further improve the performance of the SE models. Models trained using MRSD achieves the best SE performance; 
4) The best BSRNN model performs on par with or better than previous SE benchmark systems in both offline (ID 9 v.s. 14) and online (ID 15 v.s. 20) scenarios and achieves the SOTA overall performance.




% We present the best available reported numbers on the same test set from the corresponding literature of all the other systems. 
% It can be observed that when the MGD loss is not applied, BSRNN is able to outperform almost all existing systems across all evaluation metrics in both online and offline scenarios, except for the MTFAA-NET in terms of PESQ-WB. 
% After adding the MGD loss, BSRNN is able to achieve the SOTA performance on all metrics. Note that although the MGD loss is particularly designed for the PESQ-WB metric, applying the loss does not hurt all the other metrics, including the phase-sensitive SI-SNR metric.


\subsection{Personalized speech-enhancement}
Table~\ref{tab:pdns2022} provides the ablation results of the proposed system on the DNS-2022 blind test set. 
It can be observed that: 
1) The non-personalized and personalized BSRNN models show comparable performance when there is no interfering speech, while the personalized model outperforms the non-personalized model for inputs without interference speech;
2) The use of MDR discriminator loss will degrade the PDNSMOS score, one possible explanation is that the MGD loss is particularly designed for the PESQ-WB metric, which can be inconsistent with PDNSMOS; 
3) After finetuning with the MRSD discriminator loss, both models can achieve better OVRL scores on the PDNSMOS metric; 
4) The proposed model can achieve comparable or better results against previous SOTA PSE systems (ID 5 v.s. 10).  

Table~\ref{tab:pdns2023} shows the results of pBSRNN in the DNS-2023 challenge. 
Note that in this challenge, we reset the LSTM hidden representation every 10 seconds in inference.
It can be observed that:
1) The proposed system achieves better final scores than the baseline systems provided by the challenge organizer. Our model shows competitive PSE performance and ranks among top-3 in this challenge;
2) Although the proposed pBSRNN system can largely improve the human OVRL subjective evaluation scores in both tracks, the use of the proposed model can largely degrade the speech recognition word accuracy (WACC),  which indicates that current PSE models will introduce unexpected artifacts and over suppress the target speech when removing the background noise and other interfering speech.  


 




% To evalute the complexity of the online BSRNN model, we report the real-time factor (RTF) of BSRNN with Pytorch-based implementation on a MacBook Pro with Intel i5 Core to be 0.72. By applying proper model acceleration techniques, the RTF of the model can be further decreased to satisfy the requirement of computational constrained platforms or devices.
% %Under configuration on Section~\ref{sec:modelconf}, the real-time factor
% %of our online BSRNN system is about 0.72 with Python implementation (on MacBook Pro with Intel Core i5 core).
